Non-Contact Acquisition of PPG Signal using Chest Movement-Modulated Radio Signals

We present for the first time a novel method that utilizes the chest movement-modulated radio signals for non-contact acquisition of the photoplethysmography (PPG) signal. Under the proposed method, a software-defined radio (SDR) exposes the chest of a subject sitting nearby to an orthogonal frequency division multiplexing signal with 64 sub-carriers at a center frequency 5.24 GHz, while another SDR in the close vicinity collects the modulated radio signal reflected off the chest. This way, we construct a custom dataset by collecting 160 minutes of labeled data (both raw radio data as well as the reference PPG signal) from 16 healthy young subjects. With this, we first utilize principal component analysis for dimensionality reduction of the radio data. Next, we denoise the radio signal and reference PPG signal using wavelet technique, followed by segmentation and Z-score normalization. We then synchronize the radio and PPG segments using cross-correlation method. Finally, we proceed to the waveform translation (regression) task, whereby we first convert the radio and PPG segments into frequency domain using discrete cosine transform (DCT), and then learn the non-linear regression between them. Eventually, we reconstruct the synthetic PPG signal by taking inverse DCT of the output of regression block, with a mean absolute error of 8.1294. The synthetic PPG waveform has a great clinical significance as it could be used for non-contact performance assessment of cardiovascular and respiratory systems of patients suffering from infectious diseases, e.g., covid19.

==> sec5.tex <==
\section{Training and Testing of Machine Learning Classifiers}


\subsection{Data Pre-processing \& Training of Machine Learning Classifiers }  

{\it Data Pre-processing:}
We utilised a low-pass filter and a Savitzky-Golay filter to denoise the CFR extracted from the received OFDM signal, for all the experiment sessions. We inspected the whole data manually and removed artifacts where found.

{\it Training \& validation of ML classifiers: }
The Matlab's classification learner app was used to train the following ML classifiers:
K-nearest neighbour (KNN), support vector machine (SVM), decision tree (DT), ensemble classifier, and neural network. All the classifiers were trained on labelled dataset. The K-fold cross-validation strategy was used for validation in order to prevent the over-fitting issue. 

%Remember that the dataset is randomly split into smaller portions for training and testing in the cross-validation approach. For instance, if K is 5, 80 percent of the data would be used for training and the remaining 20 percent will be used for testing and validation. 
% The classifier model will train five times if K=5. 


\subsection{Performance metrics}
todo...


% \begin{table}[h!]
% \centering
% \begin{tabular}{|c| c| c| c|} 
%  \hline
%  Algorithm &
% 	Actual /Predicted&	Hydrated &	Dehydrated
% \\
% \hline

%  &	Hydrated &	\cellcolor{blue!25}73.7 & 26.3 \\
% k-NN
% (k=1) &		Dehydrated &	15.5 &	\cellcolor{blue!25}84.5  \\

% \hline 

%  &	Hydrated &	\cellcolor{blue!25}60.2 & 39.8 	 \\
% k-NN
% (k=10) &	Dehydrated&	21.9 &	\cellcolor{blue!25}78.1  \\

 
% \hline 

% 	& Hydrated &	\cellcolor{blue!25}21.1 &	78.9 \\
% k-NN
% (k=100) &	Dehydrated &	10.4 &	\cellcolor{blue!25}89.6  \\

 
%  \hline
% \end{tabular}
% \caption{Confusion matrix of k-NN algorithm for the chest movement-based method.} 
% % Total number of observations for each breathing class is 1280. }
% \label{table:knnref}
% \end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{|c| c| c| c|} 
%  \hline
%  Algorithm &
% 	Actual /Predicted&	Hydrated &	Dehydrated	
% \\
% \hline
%  &	Hydrated &	\cellcolor{blue!25}87.4 & 12.6 \\
% Linear SVM &		Dehydrated &	14.4 &	\cellcolor{blue!25}85.6  \\
 
% \hline 
%  &	Hydrated &	\cellcolor{blue!25}88.5 &	11.5 \\
% Quadratic SVM&	Dehydrated &	9.3 &	\cellcolor{blue!25}90.7 \\

% \hline 
%  &	Hydrated &	\cellcolor{blue!25}89.4 &	10.6 \\
% Cubic SVM&	Dehydrated &	7.6 &	\cellcolor{blue!25}92.4 \\

% \hline 

%  & Hydrated &	\cellcolor{blue!25}68.0 &	32.0  \\
% DT (Fine Tree) &	Dehydrated &	30.3 &	\cellcolor{blue!25}69.7 \\

%  \hline
% 	& Hydrated &	\cellcolor{blue!25}99.1 &	0.9  \\
% DT (Coarse Tree) &	Dehydrated &	83.2 &	\cellcolor{blue!25}16.3 \\

%  \hline
%%%%%%%%%%%
% Ensemble	& Hydrated &	\cellcolor{blue!25}76.2 &	23.8  \\
%  Boosted Tree &	Dehydrated &	35.6 &	\cellcolor{blue!25}64.4 \\

%  \hline
% Ensemble	& Hydrated &	\cellcolor{blue!25}82.1 &	17.9  \\
%  Bagged Tree &	Dehydrated &	26.4 &	\cellcolor{blue!25}73.6 \\

%  \hline
% Ensemble	& Hydrated &	\cellcolor{blue!25}77.9 &	22.1  \\
%  Subspace KNN &	Dehydrated &	12 &	\cellcolor{blue!25}88.0 \\

%  \hline
% Ensemble	& Hydrated &	\cellcolor{blue!25}88.9 &	11.1  \\
%  Subspace Discriminant &	Dehydrated &	9.7 &	\cellcolor{blue!25}90.3 \\

%  \hline
% %%%%%% NN
% Narrow	& Hydrated &	\cellcolor{blue!25}93.2 &	6.8  \\
%  Neural Network &	Dehydrated &	5.6 &	\cellcolor{blue!25}94.4 \\

%  \hline
%  Medium	& Hydrated &	\cellcolor{blue!25}91.4 &	8.6  \\
%  Neural Network &	Dehydrated &	6.3 &	\cellcolor{blue!25}93.7 \\

%  \hline
%  Wide & Hydrated &	\cellcolor{blue!25}91.6 &	8.4  \\
%  Neural Network &	Dehydrated &	5.8 &	\cellcolor{blue!25}94.2 \\

%  \hline
%  Bilayered	& Hydrated &	\cellcolor{blue!25}93.0 &	7.0  \\
%  Neural Network &	Dehydrated &	7.1 &	\cellcolor{blue!25}92.9 \\

%  \hline
%  Trilayered	& Hydrated &	\cellcolor{blue!25}92.8 &	7.2  \\
%  Neural Network &	Dehydrated &	93.4 &	\cellcolor{blue!25}6.6 \\

%  \hline
 
% \end{tabular}
% \caption{Confusion matrix of SVM, DT, and Ensemble classifiers for the chest movement-based method . }
% % Total number of observations for each breathing class is 1280.}
% \label{table:svmdtref}
% \end{table}

% \begin{table}[h!]
% \centering
% \begin{tabular}{|c| c|} 
%  \hline
%  Algorithm &
% 	Accuracy
% \\
% \hline
% Fine k-NN (k=1) & 79.1$\%$ \\
% Medium k-NN (k=10) & 69.2$\%$ \\
% Medium k-NN (k=100) & 55.3$\%$ \\
% \hline 
% Linear SVM & 86.5$\%$ \\
% Quadratic SVM & 89.6$\%$ \\
% Cubic SVM & 90.9$\%$ \\
% \hline 
% DT (Fine Tree) & 68.8$\%$ \\
% DT (Coarse Tree) & 58.0$\%$ \\
%  \hline
% Ensemble Boosted Tree & 70.3$\%$ \\
% Ensemble Bagged Tree & 77.9$\%$ \\
% Ensemble Subspace KNN & 82.9$\%$ \\
% Ensemble Subspace Discriminant & 89.6$\%$ \\
%  \hline
% Narrow Neural Network & 93.8$\%$ \\
% Medium Neural Network Tree & 92.5$\%$ \\
% Wide Neural Network & 92.9$\%$ \\
% Bilayered Neural Network & 93.0$\%$ \\
% Trilayered Neural Network & 93.1$\%$ \\
%  \hline
% \end{tabular}
% \caption{Performance comparison of all the classifiers for the chest movement-based method.}
% \label{table:refmoverall}
% \end{table}


\subsection{Performance comparison with the state-of-the-art}
todo ...

% \begin{table}[h!]
% \centering
% \begin{tabular}{|c| c| c| c|} 
%  \hline
%  Algorithms &
% 	Actual /Predicted&	Hydrated &	Dehydrated
% \\
% \hline
% &	Hydrated &	\cellcolor{blue!25}79.6 & 20.4 \\
% k-NN (k=1)&		Dehydrated&	14.1 &	\cellcolor{blue!25}85.9 \\

% \hline
% &	Hydrated &	\cellcolor{blue!25}69.2  & 30.8 \\
% k-NN (k=10)&		Dehydrated&	26.5&	\cellcolor{blue!25}73.5\\
% \hline
% &	Hydrated &	\cellcolor{blue!25}25.3& 74.8 \\
% k-NN (k=100)&		Dehydrated&	13& 	\cellcolor{blue!25}87.0 \\

% \hline
% &	Hydrated &	\cellcolor{blue!25}46.7 & 53.3 \\
% Linear SVM &		Dehydrated&	4.4&\cellcolor{blue!25}	95.6\\

% \hline 
% &	Hydrated&	\cellcolor{blue!25}85.3&	14.7 \\
% Quad. SVM&	Dehydrated&	7.0&	\cellcolor{blue!25}93.0 \\

% \hline 
% &	Hydrated&	\cellcolor{blue!25}87.1&	12.9 \\
% Cubic SVM&	Dehydrated&	10.6&	\cellcolor{blue!25}89.4 \\

% \hline 
% 	&Hydrated&	\cellcolor{blue!25}&	3.30 \\
% DT &	Dehydrated&	80.40&	\cellcolor{blue!25}13.12\\

%  \hline
%  &Hydrated&	\cellcolor{blue!25}91.32&	3.30 \\
% DT &	Dehydrated&	80.40&	\cellcolor{blue!25}13.12\\

%  \hline
%  Ensemble	& Hydrated &	\cellcolor{blue!25}76.2 &	23.8  \\
%  Boosted Tree &	Dehydrated &	35.6 &	\cellcolor{blue!25}64.4 \\

%  \hline
% Ensemble	& Hydrated &	\cellcolor{blue!25}82.1 &	17.9  \\
%  Bagged Tree &	Dehydrated &	26.4 &	\cellcolor{blue!25}73.6 \\

%  \hline
% Ensemble	& Hydrated &	\cellcolor{blue!25}77.9 &	22.1  \\
%  Subspace KNN &	Dehydrated &	12 &	\cellcolor{blue!25}88.0 \\

%  \hline
% Ensemble	& Hydrated &	\cellcolor{blue!25}88.9 &	11.1  \\
%  Subspace Discriminant &	Dehydrated &	9.7 &	\cellcolor{blue!25}90.3 \\

%  \hline
% %%%%%% NN
% Narrow	& Hydrated &	\cellcolor{blue!25}93.2 &	6.8  \\
%  Neural Network &	Dehydrated &	5.6 &	\cellcolor{blue!25}94.4 \\

%  \hline
%  Medium	& Hydrated &	\cellcolor{blue!25}91.4 &	8.6  \\
%  Neural Network &	Dehydrated &	6.3 &	\cellcolor{blue!25}93.7 \\

%  \hline
%  Wide & Hydrated &	\cellcolor{blue!25}91.6 &	8.4  \\
%  Neural Network &	Dehydrated &	5.8 &	\cellcolor{blue!25}94.2 \\

%  \hline
%  Bilayered	& Hydrated &	\cellcolor{blue!25}93.0 &	7.0  \\
%  Neural Network &	Dehydrated &	7.1 &	\cellcolor{blue!25}92.9 \\

%  \hline
%  Trilayered	& Hydrated &	\cellcolor{blue!25}92.8 &	7.2  \\
%  Neural Network &	Dehydrated &	93.4 &	\cellcolor{blue!25}6.6 \\

%  \hline

 
% \end{tabular}
% \caption{Confusion matrix of the three classifiers for the proposed method (hand movement-based). Total number of observations for each breathing class is 1280.}
% \label{table:confmatprop}
% \end{table}


% \begin{table}[h!]
% \centering
% \begin{tabular}{|c| c|} 
%  \hline
%  Algorithm &
% 	Accuracy
% \\
% \hline
% Fine k-NN (k=1) & 82.8$\%$ \\
% Medium k-NN (k=10) & 69.2$\%$ \\
% Medium k-NN (k=100) & 55.3$\%$ \\
% \hline 
% Linear SVM & 86.5$\%$ \\
% Quadratic SVM & 89.6$\%$ \\
% Cubic SVM & 90.9$\%$ \\
% \hline 
% DT (Fine Tree) & 68.8$\%$ \\
% DT (Coarse Tree) & 58.0$\%$ \\
%  \hline
% Ensemble Boosted Tree & 70.3$\%$ \\
% Ensemble Bagged Tree & 77.9$\%$ \\
% Ensemble Subspace KNN & 82.9$\%$ \\
% Ensemble Subspace Discriminant & 89.6$\%$ \\
%  \hline
% Narrow Neural Network & 93.8$\%$ \\
% Medium Neural Network Tree & 92.5$\%$ \\
% Wide Neural Network & 92.9$\%$ \\
% Bilayered Neural Network & 93.0$\%$ \\
% Trilayered Neural Network & 93.1$\%$ \\
%  \hline
% \end{tabular}
% \caption{Performance comparison of all the three classifiers for the proposed method (hand movement-based).}
% \label{table:propmoverall}
% \end{table}




 \begin{table}[h!]
\centering
\begin{tabular}{|c| c|} 
 \hline
 Work &
	Accuracy
\\
\hline
Liaqat et al. \cite{liaqat2022personalized} & 97.83$\%$ \\
\hline

\end{tabular}
\caption{Accuracy of ... }
\label{table:propmoverall}
\end{table}






% We presented in detail the performance results of all the classifiers for both methods (i.e., exploits the chest movement, and rhythmic hand movements). The results point towards a tradeoff: the hand movement-based method has slightly lower accuracy than the chest movement-based method (95.9\% vs. 88.1\%), but the hand movement-based method will expose the subjects to the least amount of potentially harmful radiation (full chest vs. a hand only). We further notice that the performance of the proposed methods may further be increased by implementing the state-of-the-art deep learning methods which will require a very large dataset in order to train (leading to a very extensive data collection campaign).

% A key benefit of the proposed methods is that they could lead to the development of a smart mobile health (m-health) solution that could be deployed in remote areas far away from mega cities in order to ensure the comprehensive health monitoring of the people in those areas. Additionally, the proposed method could prove to be very useful for rapid and non-contact testing of masses for their respiratory performance during the outbreak of a pandemic like covid19.


